Discrete-Time Linear-Quadratic Regulation via Optimal Transport

In this paper, we consider a discrete-time stochastic control problem with uncertain initial and target states. We first discuss the connection between optimal transport and stochastic control problems of this form. Next, we formulate a linear-quadratic regulator problem where the initial and terminal states are distributed according to specified probability densities. A closed-form solution for the optimal transport map in the case of linear-time varying systems is derived, along with an algorithm for computing the optimal map. Two numerical examples pertaining to swarm deployment demonstrate the practical applicability of the model, and performance of the numerical method.

==> notes.tex <==
\section{Optimal Transport}

\textit{Populate this when I have some time...}
\begin{itemize}
  \item Monge
  \item Kantorovic
  \item Brenier-Benamou
\end{itemize}


\section{Optimal Transport over a Linear System}


There is a nice equivalence between Brenier-Benamou mass transport and stochastic optimal control of single integrator dynamics:
\begin{align}
  \begin{array}{ll}
    \inf_{\rho,v} & \frac{1}{2}\int_{\mathbb{R}^n} \int _0^1 \|v\|_2^2 \rho dx dt\\
    \mathrm{st} & \partial_t \rho + \nabla \cdot (\rho v) = 0\\
                  & \rho(0,x) = \rho_0,~ \rho(1,x) = \rho_1
  \end{array}
 \xleftrightarrow{\mu_i \sim \rho_i(x)dx}
  \begin{array}{ll}
    \inf_v & \frac{1}{2}\mathbb{E} \left[ \int_0^1 \|v(t,x^v)\|_2^2 dt \right]\\
    \mathrm{st} & \dot{x}^v = v(t,x^v(t))\\
           & x^v(0) \sim \mu_0,~x^v(1) \sim\mu.
  \end{array}
\end{align}

Let's discuss the solutions in the single-integrator case, and then the LTV case.

\subsection{Single-Integrator Dynamics}

The solution to the above problems is given by
\begin{align}
  \rho(t,x) &= \dfrac{d \mu_t}{dx}\\
  v(t,x) &= T \circ T_t^{-1} - T_t^{-1} (x),
\end{align}
where
\begin{align}
  T_t(x) &= (1-t)x + tT(x)\\
  \mu_t &= (T_t)_{\#} \mu_0,
\end{align}
and $T(x)$ is the Monge map from $\mu_0$ to $\mu_1$ under quadratic cost.

\subsection{LTV Dynamics}

The OMT problem with prior dynamics is given as\cite{Chen2017}
\begin{align}
  \begin{array}{ll}
    \inf_{\rho,u} & \frac{1}{2}\int_{\mathbb{R}^n} \int _0^1 \|u\|_2^2 \rho dx dt\\
    \mathrm{st} & \partial_t \rho + \nabla \cdot (\rho (A(t) x(t) + B(t) u(t)) = 0\\
                  & \rho(0,x) = \rho_0,~ \rho(1,x) = \rho_1.
  \end{array}  
\end{align}
Note that the cost of this problem is simply
\begin{align}
\frac{1}{2} \mathbb{E} \left[ \int_0^1 \|v(t,x^v)\|_2^2 dt \right],
\end{align}
and one can write
\begin{align} 
  c(x,y) &= \frac{1}{2} (y- \Phi_{10})^T M_{10}^{-1} (y- \Phi_{10}),
\end{align}
where
\begin{align}
  M_{10} = \int_0^1 \Phi(1,\tau) B(\tau)B(\tau)^T \Phi(1,\tau) d\tau,
\end{align}
and $\Phi(t,s)$ is the state transition matrix of the dynamics.
Under the coordinate transformation
\begin{align}
  \begin{bmatrix}
    x \\ y
  \end{bmatrix}\mapsto
  \begin{bmatrix}
    \hat{x} \\ \hat{y}
  \end{bmatrix}\triangleq
  \begin{bmatrix}
    M_{10}^{-1/2} \Phi(1,0) x\\
    M_{10}^{-1/2} y
  \end{bmatrix},
\end{align}
the cost can be written as the cost of the Kantorovic OT problem with coupling $\pi$:
\begin{align}
\frac{1}{2}\mathbb{E}\left[ c(x,y) \right] &= \frac{1}{2} \mathbb{E} \left[ \int_0^1 \|v(t,x^v)\|_2^2 dt \right]\\
                                           &= \frac{1}{2} \mathbb{E} \left[  \frac{1}{2} (y- \Phi_{10})^T M_{10}^{-1} (y- \Phi_{10}) \right]\\
                                           &= \frac{1}{2} \int_{\mathbb{R}^n\times \mathbb{R}^n} \|\hat{y} - \hat{x} \|_2^2 \pi(dx,dy).
\end{align}
The Monge map of the problem in the last display can be then used to construct the optimal control as in the single integrator case.

Do this for discrete mass transport.


\section{Discrete Mass Transport}

Recall the continuous-time Brenier-Benamou problem:
\begin{align}
    \begin{array}{ll}
    \inf_{\rho,u} & \frac{1}{2}\int_{\mathbb{R}^n} \int _0^1 \|u(t,x)\|_2^2 \rho(t,x) dx dt\\
    \mathrm{st} & \partial_t \rho + \nabla \cdot (\rho (A(t) x(t) + B(t) u(t)) = 0\\
                  & \rho(0,x) = \rho_0,~ \rho(1,x) = \rho_1.
  \end{array}  
\end{align}

This was shown to be equivalent to the discrete one-step Monge problem.
In control, however, we want to be able to actuate inputs over many timesteps.
Krishnan and Martinez discusses multi-stage optimal transport:
\begin{align}
C(\mu_0,\mu_T) &= \min_{\substack{(\mu_1,\dots,\mu_T) \\ \mu_k \in \mathcal{P}(\Omega) }} \sum_{k=1}^{t_f} C(\mu_{k-1}, \mu_k).
\end{align}
Insertez les details.
I want to use this, and the discrete state transition matrix, to compute the discrete time mass transport.


\subsection{Connection to Optimal Control}

Consider the problem 
\begin{align}
  \begin{array}{ll}
    \min_{u} & \sum_{t=0}^{t_f-1} \|u(t)\|_2^2\\
    \mathrm{s.t.} & x(k+1) = Ax(k) + Bu(k)\\
             & x(0) = x,~x(t_f) = y.
  \end{array}\label{eq:1}
\end{align}
Chen \emph{et al.} discusses the continuous-time version of this problem and its connections to mass transport\cite{Chen2017}. 
Here, we derive the discrete-time version.
To solve Problem~\eqref{eq:1}, note that we want
\begin{align}
y =   x(t_f) &= A^\intercal x(0) + \mathcal{C}_{t_f}
\begin{bmatrix}
  u(t_f-1) \\ \vdots \\ u(0),
\end{bmatrix}
\end{align}
or in other words we want
\begin{align}
 y-  A^\intercal x(0) \in \mathcal{R}_{t_f},
\end{align}
where $\mathcal{R}_{t_f}$ is the reachable set from the origin in $t_f$ steps.
We can therefore write the solution of Problem~\eqref{eq:1} as
\begin{align}
  \mathrm{arg~min}\sum_{t=0}^{t_f} \|u(t)\|_2^2 &=  \mathrm{arg~min}\left\|
\begin{bmatrix}
  u^*(t_f-1)\\\vdots\\u^*(0)
\end{bmatrix}
\right\|_2^2\\
                                                &= \mathcal{C}_{t_f}^\intercal \left(\mathcal{C}_{t_f} \mathcal{C}_{t_f}^\intercal \right)^{-1} ( y - A^{t_f-1} x),
\end{align}
or as 
\begin{align}
  u^*(t) &= B^\intercal (A^\intercal)^{t_f - 1 - t} W(0,t_f)^{-1}( y - A^{t_f-1} x) \\
  W(0,t_f) &= \sum_{k=0}^{t_f-1} A^k BB^\intercal (A^\intercal)^k,
\end{align}
and similarly the minimum cost is
\begin{align}
  \min \sum_{t=0}^{t_f} \|u(t)\|_2^2 &= \left\|
\begin{bmatrix}
  u^*(t_f-1)\\\vdots\\u^*(0)
\end{bmatrix}
\right\|_2^2\\
                                                &= \| \mathcal{C}_{t_f}^\intercal \left(\mathcal{C}_{t_f} \mathcal{C}_{t_f}^\intercal \right)^{-1} ( y - A^{t_f-1} x)\|_2^2\\
                                     &= ( y - A^{t_f-1} x)^T W(0,t_f)^{-1} ( y - A^{t_f-1} x).
\end{align}
Under the coordinate transformation
\begin{align}
  \begin{bmatrix}
    x \\ y
  \end{bmatrix}\mapsto
  \begin{bmatrix}
    \hat{x} \\ \hat{y}
  \end{bmatrix}\triangleq
  \begin{bmatrix}
    W(0,t_f)^{-1/2} A^{t_f-1} x\\
    W(0,t_f)^{-1/2} y
  \end{bmatrix},
\end{align}
we can equate the two problems
\marginnote{Write the Kantorovich problem properly!}
\begin{align}
  \begin{array}{ll}
    \min & \mathbb{E} \left[ \sum_{t=0}^{t_f} \|u(t)\|_2^2 \right]\\
    \mathrm{s.t.} & x(0) \sim \mu_0,~x(t_f) \sim \mu_{t_f}
  \end{array} \leftrightarrow
  \begin{array}{ll}
    \min_{T} & \int_{\mathbb{R}^n\times \mathbb{R}^n} \|\hat{y} - \hat{x} \|_2^2 \pi(dx,dy)\\
    \mathrm{s.t.} & x(0) \sim \mu_0,~x(t_f) \sim \mu_{t_f}\\
             & T_{\#}\mu_0 = \mu_{1}
  \end{array}
\end{align}
since
\begin{align}
   \mathbb{E}_{\mu_0} \left[ \sum_{t=0}^{t_f} \|u(t)\|_2^2 \right] &= \mathbb{E}_{\mu_0} \left[  ( y - A^{t_f-1} x)^T W(0,t_f)^{-1} ( y - A^{t_f-1} x) \right]\\
                                                           &= \mathbb{E}_{\mu_0} \left[ \|\hat{x} - \hat{y}\|_2^2 \right].
\end{align}
Noting that the minimizer of the Kantorovich dual is the same as for Monge, we can establish the equivalence of the problems.
\marginnote{I really need to clean this up, this isn't at all rigorous}

After cleaning this up, we can see that
\begin{align}
  C(\mu_0,\mu_{t_f})  &=
\begin{array}{ll}
  \min & \mathbb{E}_{\mu_0} \left[ \|\hat{x} - \hat{y}\|_2^2 \right]\\
  \mathrm{s.t.} & 
\end{array}\\
                      &= \mathbb{E}_{\mu_0} \left[  ( y - A^{t_f-1} x)^T W(0,t_f)^{-1} ( y - A^{t_f-1} x) \right]\\
                      &= \mathbb{E}_{\mu_0} \left[ \sum_{t=0}^{t_f} \|u(t) \|_2^2 \right]\\
\end{align}

==> old-examples.tex <==
\section{EXAMPLES}
\label{sec:examples}

In this section, we provide numerical experiments of the results in \S\ref{sec:results}.


\subsection{2D LQR Example}
First, we provide an example of the numerical implementation of Theorem~\ref{thr:1}.
We implemented the optimal transport method for LQR on a 2-state, 1-input system with matrices
\begin{align}
    A = \begin{bmatrix}
   0.9& -0.1 \\
         -0.1 & 0.8          
        \end{bmatrix},~ B = 
  \begin{bmatrix}
      1 \\ 0
  \end{bmatrix}\\
  Q_k = I_2,~R_k=1,~0\leq k \leq 10.
\end{align}
Let the states be denoted by $z_k:=(z_k^{(1)},z_k^{(2)})$.
Our initial states were distributed according to $\rho_0(x)$ depicted in Fig.~\ref{fig:eg1dist}, and we sought to steer the system to the distribution $\rho_1(y)$, also depicted in Fig.~\ref{fig:eg1dist}.

The distributions $\rho_0,\rho_1$ are supported on a discrete grid on the cube $[-1,1]^2$ with a discretization length $\Delta x = \Delta y = 0.0588$.
The optimal transport map $T^*$ was computed by solving \eqref{eq:27} discretized on this grid, with a cost matrix $C$ computed using \eqref{eq:23} from Lemma~\ref{lem:1}.
In Fig.~\ref{fig:eg1map}, we show a color map of the image of $T^*$.
On the left is the coordinate in the first dimension as a function of the initial $(x^{(1)},x^{(2)}) = (z_{0}^{(1)},z_0^{(2)})$, and on the right is the coordinate in the second dimension as a function of the initial $(z_{0}^{(1)},z_0^{(2)})$.
One can note that the numerical approximation contains outliers in regions where $\bmrho_0$ has little mass.

We ran an experiment with 10,000 i.i.d.~random initial conditions sampled from $\rho_0$.
For each initial condition $z_0$, the optimal map computed the corresponding final condition as $z_{t_f} = T^*(z_0)$.
The simulation then used the optimal control inputs~\eqref{eq:26} to guide the system to $T^*(z_0)$ over a time horizon of $0\leq k \leq 10$.
Plots of the empirical distributions are shown in Fig.~\ref{fig:eg1emp} at times $t=0,3,7,10$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./figs/example_1_density.eps}
    \caption{True distribitions of the initial (left: $\rho_0(x)$) and target (right: $\rho_1(x)$) states.}
    \label{fig:eg1dist}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./figs/example_1_maps.eps}
    \caption{Images of the optimal map $T^*(x)$ in the $y^{(1)}$ (left) and $y^{(2)}$ (right) coordinates of the target domain. Note that the map is numerically less accurate in regions where $\bmrho_0(x)$ has small mass, such as the white square.}
    \label{fig:eg1map}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./figs/example_1_states.eps}
    \caption{Empirical distributions of the states of the system over time. Top left: $t=0$. Top right: $t=3$. Bottom left: $t=7$. Bottom right: $t=10$.}
    \label{fig:eg1emp}
\end{figure}


\subsection{Swarm Deployment}

Consider the task of assigning target positions to $n$ agents whose initial states have an empirical distribution approximating $\rho_0(x)dx$, but not randomly instantiated.
For example, consider $n$ agents spaced at constant intervals in the cube $[-1,1]^2$, as depicted in the middle-left subfigure of Fig.~\ref{fig:eg2dist}.
Clearly, this is an approximation of a uniform distribution.
Our target distribution is the logo of the Swiss Federal Institute of Technology, Z\"{u}rich, discretized over a $35\times 35$ pixel domain.
A target application could be a swarm of UAVs providing a background performance act during a university event.

Using discrete single-integrator dynamics
\begin{align}
\begin{split}
  &A_k = Q_k = R_k= I_2,~0\leq k \leq 10,\\
  &B_k = I_2,~0\leq k \leq 5,~B_k = \mathbf{0}_{2\times 2},~5<k\leq 10.
\end{split}\label{eq:29}
\end{align}
we compute the optimal map using~\eqref{eq:27} with the cost matrix~\eqref{eq:23} from Lemma~\ref{lem:1}, depicted in Figure~\ref{fig:eg2map}.
The simulation was again produced over a time horizon of $0\leq k \leq 10$.
This time, we plot the explicit mapping between points in a grid and their target states as generated by the map $T^*$, as shown in the bottom-right of Figure~\ref{fig:eg2map}.

The dynamics~\eqref{eq:29} are controllable, in the sense that the controllability gramian~\eqref{eq:28} $W_c(t_f,0)$ is positive-definite, however the matrix $S_2$ in \label{eq:20} is $\mathbf{0}_{4\times2}$.
Since $\mathbf{0}_{4\times 2}^\dag = \mathbf{0}_{2\times 4}$, by \eqref{eq:20}, this simply means that the control is zero for $6\leq k \leq 10$.
As the system is controllable, it is steered to the final position by timestep $k=5$, as evident in Figure~\ref{fig:lqr}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{./figs/control_lqr.eps}
  \caption{Top: Trajectory of dynamics \eqref{eq:29}. Bottom: Control computed by solving \eqref{eq:24} using \texttt{cvx}\cite{cvx} (solid line) and via \eqref{eq:22} (markers). Red (black) dashed lines indicate target (initial) states.}
  \label{fig:lqr}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./figs/example_2_density.eps}
    \caption{Top: plots of the initial uniform distribution (left), and target distribution representing the ETH logo (right). 
Middle: Initial conditions $(x,y)$ uniformly spaced in $[-1,1]^2$ (left), and their corresponding terminal conditions $T^*(x,y)$ (right).
Bottom: empirical distribution of the terminal states from the middle-right, and a plot showing the corresponding final states interpolated from an initial state.}
    \label{fig:eg2dist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./figs/example_2_maps.eps}
    \caption{Images of the optimal map $T^*(x)$ in the $x$ (left) and $y$ (right) coordinates of the target domain. }
    \label{fig:eg2map}
\end{figure}

%%% Local Variables:
%%% TeX-master: "cdc-lqr-ot.tex"
%%% End:

==> old_work.tex <==
\subsection{OT \& LQR}
\textcolor{blue}{We will probably have to remove this section}
Consider the OT problem with dynamical constraints:
\begin{align}
  \begin{array}{ll}
    \min_{T_k} & \sum_{k=1}^N \int \|x_k - T(x_k)\|^2 d\mu_k\\
    \mathrm{s.t.} & x_k \sim \mu_k\\
               & \mu_{k\#} T_k = \mu_{k+1}\\
               & T_k(x_k) = A_k x_k + B_k u_k
  \end{array} \tag{P4} \label{eq:1}
\end{align}
\begin{theorem}
  Problem~\eqref{eq:1} is equivalent to the stochastic LQR formulation,
  \begin{align}
    \begin{array}{ll}
      \min_{u_k} & \sum_{k=1}^N \mathbf{E}_{\mu_k} \left[ x_k^TQ_k x_k + u_k^T R_k u_k +2 x_k^T N_k u_k\right]\\
                 & \mu_{k\#} T_k = \mu_{k+1}.
    \end{array}
  \end{align}
  under the following idenfitications
  \begin{align}
    Q_k = (I-A_k)^T(I-A_k),~R_k = B_k^TB_k,~N_k = (A_k - I)^T B_k.
  \end{align}
\end{theorem}
\begin{proof}
  The argument of the integral in the cost in Problem~\eqref{eq:1} can be written as
  \begin{align}
    & \sum_{k=1}^N\|x_k - T(x_k)\|^2  = \sum_{k=1}^N \| x_k - (A_k x_k + B_k u_k ) \|^2 \\
    =& \sum_{k=1}^N \left\{ \left(x_k - (A_k x_k - B_k u_k)\right)^T \left(x_k - (A_k x_k - B_k u_k)\right) \right\}\\
    =& \sum_{k=1}^N \left\{x_k^T (I-A_k)^T(I-A_k)x_k + u_k^T B_k^T B_k u_k - 2x_k^T (I-A_k)^T B_k u_k \right\}\\
    \triangleq & \sum_{k=1}^N \left\{x_k^TQ_k x_k + u_k^T R_k u_k +2 x_k^T N_k u_k\right\},
  \end{align}
  and so
  \begin{align}
   & \sum_{k=1}^N \int \|x_k - T(x_k)\|^2 d\mu_k \\
    =&  \sum_{k=1}^N \int \left\{x_k^TQ_k x_k + u_k^T R_k u_k +2 x_k^T N_k u_k\right\} d\mu_k\\
    =& \sum_{k=1}^N \mathbf{E}_{\mu_k} \left[ x_k^TQ_k x_k + u_k^T R_k u_k +2 x_k^T N_k u_k\right].
  \end{align}
\end{proof}
The optimal one-step Monge map between two Gaussians $N(m_k,\Sigma_k),N(m_{k+1},\Sigma_{k+1})$ is a scaling and a translation. 
Is that the case here? I.e., can we set
\begin{align}
  x_k \mapsto m_{k+1} + \tilde{A}_k(x_k - m_k) = A_k x_k + B_k u_k,
\end{align}
where
\begin{align}
  \tilde{A}_k \triangleq \Sigma_k ^{-1/2} \left( \Sigma_k^{1/2} \Sigma_{k+1} \Sigma_k \right)^{1/2} \Sigma_k^{1/2}
\end{align}
Probably not, some sort of Ricatti recursion will happen.
